Measurement of the fluctuations in the number of muons in extensive air showers with the Pierre Auger Observatory

We present the first measurement of the fluctuations in the number of muons in extensive air showers produced by ultrahigh energy cosmic rays. We find that the measured fluctuations are in good agreement with predictions from air shower simulations. This observation provides new insights into the origin of the previously reported deficit of muons in air shower simulations and constrains models of hadronic interactions at ultrahigh energies. Our measurement is compatible with the muon deficit originating from small deviations in the predictions from hadronic interaction models of particle production that accumulate as the showers develop.

==> author_list_latex.tex <==
% created on 2020-07-29, added Hans, Ines and Guillermo

\author{A.~Aab}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Abreu}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Aglietta}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{J.M.~Albury}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{I.~Allekotte}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.~Almela}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{J.~Alvarez-Mu\~niz}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{R.~Alves Batista}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{G.A.~Anastasi}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{L.~Anchordoqui}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{B.~Andrada}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{S.~Andringa}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.~Aramo}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{P.R.~Ara\'ujo Ferreira}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.~Asorey}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Assis}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Avila}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{A.M.~Badescu}
\affiliation{University Politehnica of Bucharest, Bucharest, Romania}

\author{A.~Bakalova}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Balaceanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{F.~Barbato}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{R.J.~Barreira Luz}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{K.H.~Becker}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.A.~Bellido}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Berat}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{M.E.~Bertaina}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{X.~Bertou}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.L.~Biermann}
\affiliation{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}

\author{T.~Bister}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{J.~Biteau}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{J.~Blazek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Bleve}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{M.~Boh\'a\v{c}ov\'a}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{D.~Boncioli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{C.~Bonifazi}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{L.~Bonneau Arbeletche}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{N.~Borodai}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.M.~Botti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Brack}
\affiliation{Colorado State University, Fort Collins, CO, USA}

\author{T.~Bretz}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{F.L.~Briechle}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{P.~Buchholz}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{A.~Bueno}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{S.~Buitink}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Buscemi}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{K.S.~Caballero-Mora}
\affiliation{Universidad Aut\'onoma de Chiapas, Tuxtla Guti\'errez, Chiapas, M\'exico}

\author{L.~Caccianiga}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{A.~Cancio}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{F.~Canfora}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{I.~Caracas}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.M.~Carceller}
\affiliation{Universidad de Granada and C.A.F.P.E., Granada, Spain}

\author{R.~Caruso}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{A.~Castellina}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{F.~Catalani}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{G.~Cataldi}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.~Cazon}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Cerda}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{J.A.~Chinellato}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{K.~Choi}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{J.~Chudoba}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{L.~Chytka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{R.W.~Clay}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.C.~Cobos Cerutti}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{R.~Colalillo}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{A.~Coleman}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}

\author{M.R.~Coluccia}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{R.~Concei\c{c}\~ao}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{A.~Condorelli}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{G.~Consolati}
\affiliation{INFN, Sezione di Milano, Milano, Italy}
\affiliation{Politecnico di Milano, Dipartimento di Scienze e Tecnologie Aerospaziali , Milano, Italy}

\author{F.~Contreras}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{F.~Convenga}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{C.E.~Covault}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}
\affiliation{also at Radboud Universtiy Nijmegen, Nijmegen, The Netherlands}

\author{S.~Dasso}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}
\affiliation{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires and CONICET, Buenos Aires, Argentina}

\author{K.~Daumiller}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{B.R.~Dawson}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.A.~Day}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{R.M.~de Almeida}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{J.~de Jes\'us}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{S.J.~de Jong}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{G.~De Mauro}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.R.T.~de Mello Neto}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.~De Mitri}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{J.~de Oliveira}
\affiliation{Universidade Federal Fluminense, EEIMVR, Volta Redonda, RJ, Brazil}

\author{D.~de Oliveira Franco}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{V.~de Souza}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{E.~De Vito}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{J.~Debatin}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{M.~del R\'\i{}o}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{O.~Deligny}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{H.~Dembinski}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{N.~Dhital}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Di Matteo}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{C.~Dobrigkeit}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{J.C.~D'Olivo}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{R.C.~dos Anjos}
\affiliation{Universidade Federal do Paran\'a, Setor Palotina, Palotina, Brazil}

\author{M.T.~Dova}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{J.~Ebr}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{R.~Engel}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{I.~Epicoco}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{M.~Erdmann}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{C.O.~Escobar}
\affiliation{Fermi National Accelerator Laboratory, USA}

\author{A.~Etchegoyen}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{H.~Falcke}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{J.~Farmer}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{G.~Farrar}
\affiliation{New York University, New York, NY, USA}

\author{A.C.~Fauth}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{N.~Fazzini}
\affiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{F.~Feldbusch}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Fenu}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{B.~Fick}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{J.M.~Figueira}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Filip\v{c}i\v{c}}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{T.~Fodran}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.M.~Freire}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{T.~Fujii}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}
\affiliation{now at Hakubi Center for Advanced Research and Graduate School of Science, Kyoto University, Kyoto, Japan}

\author{A.~Fuster}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Buenos Aires, Argentina}

\author{C.~Galea}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{C.~Galelli}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{B.~Garc\'\i{}a}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Mendoza, Argentina}

\author{A.L.~Garcia Vegas}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.~Gemmeke}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{F.~Gesualdi}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Gherghel-Lascu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{P.L.~Ghia}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{U.~Giaccari}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Giammarchi}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{M.~Giller}
\affiliation{University of \L{}\'od\'z, Faculty of Astrophysics, \L{}\'od\'z, Poland}

\author{J.~Glombitza}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{F.~Gobbi}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{F.~Gollan}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{G.~Golup}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{M.~G\'omez Berisso}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{P.F.~G\'omez Vitale}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{J.P.~Gongora}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{N.~Gonz\'alez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{I.~Goos}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{D.~G\'ora}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{A.~Gorgi}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Gottowik}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{T.D.~Grubb}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{F.~Guarino}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{G.P.~Guedes}
\affiliation{Universidade Estadual de Feira de Santana, Feira de Santana, Brazil}

\author{E.~Guido}
\affiliation{INFN, Sezione di Torino, Torino, Italy}
\affiliation{Universit\`a Torino, Dipartimento di Fisica, Torino, Italy}

\author{S.~Hahn}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{R.~Halliday}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{M.R.~Hampel}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{P.~Hansen}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{D.~Harari}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{V.M.~Harvey}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Haungs}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{T.~Hebbeker}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{D.~Heck}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{G.C.~Hill}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{C.~Hojvat}
\affiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{J.R.~H\"orandel}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}

\author{P.~Horvath}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Hrabovsk\'y}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{T.~Huege}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{J.~Hulsman}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Insolia}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{P.G.~Isar}
\affiliation{Institute of Space Science, Bucharest-Magurele, Romania}

\author{J.A.~Johnsen}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{J.~Jurysek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~K\"a\"ap\"a}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{K.H.~Kampert}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Keilhauer}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{J.~Kemp}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{H.O.~Klages}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Kleifges}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{J.~Kleinfeller}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~K\"opke}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{G.~Kukec Mezek}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{B.L.~Lago}
\affiliation{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Nova Friburgo, Brazil}

\author{D.~LaHurd}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{R.G.~Lang}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{N.~Langner}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{M.A.~Leigui de Oliveira}
\affiliation{Universidade Federal do ABC, Santo Andr\'e, SP, Brazil}

\author{V.~Lenok}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~Letessier-Selvon}
\affiliation{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Sorbonne Universit\'e, Universit\'e de Paris, CNRS-IN2P3, Paris, France}

\author{I.~Lhenry-Yvon}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{D.~Lo Presti}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{L.~Lopes}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{R.~L\'opez}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{R.~Lorek}
\affiliation{Case Western Reserve University, Cleveland, OH, USA}

\author{Q.~Luce}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{A.~Lucero}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.P.~Lundquist}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{A.~Machado Payeras}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}

\author{G.~Mancarella}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{D.~Mandat}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{B.C.~Manning}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{J.~Manshanden}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{P.~Mantsch}
\affiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{S.~Marafico}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{A.G.~Mariazzi}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{I.C.~Mari\c{s}}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{G.~Marsella}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{D.~Martello}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Martinez}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, SP, Brazil}

\author{O.~Mart\'\i{}nez Bravo}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.~Mastrodicasa}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.J.~Mathes}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{J.~Matthews}
\affiliation{Louisiana State University, Baton Rouge, LA, USA}

\author{G.~Matthiae}
\affiliation{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Roma, Italy}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{E.~Mayotte}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{P.O.~Mazur}
\affiliation{Fermi National Accelerator Laboratory, Fermilab, Batavia, IL, USA}

\author{G.~Medina-Tanco}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{D.~Melo}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Menshikov}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{K.-D.~Merenda}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{S.~Michal}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.I.~Micheletti}
\affiliation{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Rosario, Argentina}

\author{L.~Miramonti}
\affiliation{Universit\`a di Milano, Dipartimento di Fisica, Milano, Italy}
\affiliation{INFN, Sezione di Milano, Milano, Italy}

\author{S.~Mollerach}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{F.~Montanet}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{C.~Morello}
\affiliation{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Mostaf\'a}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{A.L.~M\"uller}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.A.~Muller}
\affiliation{Universidade Estadual de Campinas, IFGW, Campinas, SP, Brazil}
\affiliation{also at Universidade Federal de Alfenas, Po\c{c}os de Caldas, Brazil}
\affiliation{Universidade Federal do Rio de Janeiro, Instituto de F\'\i{}sica, Rio de Janeiro, RJ, Brazil}

\author{K.~Mulrey}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{R.~Mussa}
\affiliation{INFN, Sezione di Torino, Torino, Italy}

\author{M.~Muzio}
\affiliation{New York University, New York, NY, USA}

\author{W.M.~Namasaka}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{L.~Nellen}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{M.~Niculescu-Oglinzanu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{M.~Niechciol}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{D.~Nitz}
\affiliation{Michigan Technological University, Houghton, MI, USA}
\affiliation{also at Karlsruhe Institute of Technology, Karlsruhe, Germany}

\author{D.~Nosek}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{V.~Novotny}
\affiliation{Charles University, Faculty of Mathematics and Physics, Institute of Particle and Nuclear Physics, Prague, Czech Republic}

\author{L.~No\v{z}ka}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{A Nucita}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{L.A.~N\'u\~nez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{M.~Palatka}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Pallotta}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{P.~Papenbreer}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{G.~Parente}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Parra}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{M.~Pech}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Pedreira}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{J.~P\c{e}kala}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{R.~Pelayo}
\affiliation{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico, D.F., M\'exico}

\author{J.~Pe\~na-Rodriguez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{J.~Perez Armand}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{M.~Perlin}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{L.~Perrone}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{S.~Petrera}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{T.~Pierog}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Pimenta}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{V.~Pirronello}
\affiliation{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Catania, Italy}
\affiliation{INFN, Sezione di Catania, Catania, Italy}

\author{M.~Platino}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{B.~Pont}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{M.~Pothast}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{P.~Privitera}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{M.~Prouza}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{A.~Puyleart}
\affiliation{Michigan Technological University, Houghton, MI, USA}

\author{S.~Querchfeld}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Rautenberg}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{D.~Ravignani}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Reininghaus}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~Ridky}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Riehn}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{M.~Risse}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{P.~Ristori}
\affiliation{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Villa Martelli, Argentina}

\author{V.~Rizi}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{W.~Rodrigues de Carvalho}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{J.~Rodriguez Rojo}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{M.J.~Roncoroni}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Roth}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{E.~Roulet}
\affiliation{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), San Carlos de Bariloche, Argentina}

\author{A.C.~Rovero}
\affiliation{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Buenos Aires, Argentina}

\author{P.~Ruehl}
\affiliation{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Siegen, Germany}

\author{S.J.~Saffi}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{A.~Saftoiu}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{F.~Salamida}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{H.~Salazar}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{G.~Salina}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.D.~Sanabria Gomez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{F.~S\'anchez}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{E.M.~Santos}
\affiliation{Universidade de S\~ao Paulo, Instituto de F\'\i{}sica, S\~ao Paulo, SP, Brazil}

\author{E.~Santos}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.~Sarazin}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{R.~Sarmento}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{C.~Sarmiento-Cano}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{R.~Sato}
\affiliation{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Malarg\"ue, Argentina}

\author{P.~Savina}
\affiliation{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Lecce, Italy}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}
\affiliation{CNRS/IN2P3, IJCLab, Universit\'e Paris-Saclay, Orsay, France}

\author{C.M.~Sch\"afer}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{V.~Scherini}
\affiliation{INFN, Sezione di Lecce, Lecce, Italy}

\author{H.~Schieler}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Schimassek}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Schimp}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{F.~Schl\"uter}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~Schmidt}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{O.~Scholten}
\affiliation{KVI -- Center for Advanced Radiation Technology, University of Groningen, Groningen, The Netherlands}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{P.~Schov\'anek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{F.G.~Schr\"oder}
\affiliation{University of Delaware, Department of Physics and Astronomy, Bartol Research Institute, Newark, DE, USA}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{S.~Schr\"oder}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{J.~Schulte}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{S.J.~Sciutto}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{M.~Scornavacche}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{R.C.~Shellard}
\affiliation{Centro Brasileiro de Pesquisas Fisicas, Rio de Janeiro, RJ, Brazil}

\author{G.~Sigl}
\affiliation{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Hamburg, Germany}

\author{G.~Silli}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{O.~Sima}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}
\affiliation{also at University of Bucharest, Physics Department, Bucharest, Romania}

\author{R.~\v{S}m\'\i{}da}
\affiliation{University of Chicago, Enrico Fermi Institute, Chicago, IL, USA}

\author{P.~Sommers}
\affiliation{Pennsylvania State University, University Park, PA, USA}

\author{J.F.~Soriano}
\affiliation{Department of Physics and Astronomy, Lehman College, City University of New York, Bronx, NY, USA}

\author{J.~Souchard}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{R.~Squartini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{M.~Stadelmaier}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{D.~Stanca}
\affiliation{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Bucharest-Magurele, Romania}

\author{S.~Stani\v{c}}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{J.~Stasielak}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{P.~Stassi}
\affiliation{Univ.\ Grenoble Alpes, CNRS, Grenoble Institute of Engineering Univ.\ Grenoble Alpes, LPSC-IN2P3, 38000 Grenoble, France, France}

\author{A.~Streich}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{M.~Su\'arez-Dur\'an}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{T.~Sudholz}
\affiliation{University of Adelaide, Adelaide, S.A., Australia}

\author{T.~Suomij\"arvi}
\affiliation{Universit\'e Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France, France}

\author{A.D.~Supanitsky}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{J.~\v{S}up\'\i{}k}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{Z.~Szadkowski}
\affiliation{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics,\L{}\'od\'z, Poland}

\author{A.~Taboada}
\affiliation{Karlsruhe Institute of Technology, Institute for Experimental Particle Physics (ETP), Karlsruhe, Germany}

\author{A.~Tapia}
\affiliation{Universidad de Medell\'\i{}n, Medell\'\i{}n, Colombia}

\author{C.~Timmermans}
\affiliation{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Science Park, Amsterdam, The Netherlands}
\affiliation{IMAPP, Radboud University Nijmegen, Nijmegen, The Netherlands}

\author{O.~Tkachenko}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{P.~Tobiska}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.J.~Todero Peixoto}
\affiliation{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Lorena, SP, Brazil}

\author{B.~Tom\'e}
\affiliation{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Lisboa, Portugal}

\author{G.~Torralba Elipe}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{A.~Travaini}
\affiliation{Observatorio Pierre Auger, Malarg\"ue, Argentina}

\author{P.~Travnicek}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{C.~Trimarelli}
\affiliation{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{M.~Trini}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{M.~Tueros}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{R.~Ulrich}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{M.~Unger}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{L.~Vaclavek}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{M.~Vacula}
\affiliation{Palacky University, RCPTM, Olomouc, Czech Republic}

\author{J.F.~Vald\'es Galicia}
\affiliation{Universidad Nacional Aut\'onoma de M\'exico, M\'exico, D.F., M\'exico}

\author{I.~Vali\~no}
\affiliation{Gran Sasso Science Institute, L'Aquila, Italy}
\affiliation{INFN Laboratori Nazionali del Gran Sasso, Assergi (L'Aquila), Italy}

\author{L.~Valore}
\affiliation{Universit\`a di Napoli ``Federico II'', Dipartimento di Fisica ``Ettore Pancini'', Napoli, Italy}
\affiliation{INFN, Sezione di Napoli, Napoli, Italy}

\author{E.~Varela}
\affiliation{Benem\'erita Universidad Aut\'onoma de Puebla, Puebla, M\'exico}

\author{V.~Varma K.C.}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{A.~V\'asquez-Ram\'\i{}rez}
\affiliation{Universidad Industrial de Santander, Bucaramanga, Colombia}

\author{D.~Veberi\v{c}}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{C.~Ventura}
\affiliation{Universidade Federal do Rio de Janeiro (UFRJ), Observat\'orio do Valongo, Rio de Janeiro, RJ, Brazil}

\author{I.D.~Vergara Quispe}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{V.~Verzi}
\affiliation{INFN, Sezione di Roma ``Tor Vergata'', Roma, Italy}

\author{J.~Vicha}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{J.~Vink}
\affiliation{Universiteit van Amsterdam, Faculty of Science, Amsterdam, The Netherlands}

\author{S.~Vorobiov}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{H.~Wahlberg}
\affiliation{IFLP, Universidad Nacional de La Plata and CONICET, La Plata, Argentina}

\author{A.A.~Watson}
\affiliation{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}

\author{M.~Weber}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik, Karlsruhe, Germany}

\author{A.~Weindl}
\affiliation{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik, Karlsruhe, Germany}

\author{L.~Wiencke}
\affiliation{Colorado School of Mines, Golden, CO, USA}

\author{H.~Wilczy\'nski}
\affiliation{Institute of Nuclear Physics PAN, Krakow, Poland}

\author{T.~Winchen}
\affiliation{Vrije Universiteit Brussels, Brussels, Belgium}

\author{M.~Wirtz}
\affiliation{RWTH Aachen University, III.\ Physikalisches Institut A, Aachen, Germany}

\author{D.~Wittkowski}
\affiliation{Bergische Universit\"at Wuppertal, Department of Physics, Wuppertal, Germany}

\author{B.~Wundheiler}
\affiliation{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Buenos Aires, Argentina}

\author{A.~Yushkov}
\affiliation{Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic}

\author{O.~Zapparrata}
\affiliation{Universit\'e Libre de Bruxelles (ULB), Brussels, Belgium}

\author{E.~Zas}
\affiliation{Instituto Galego de F\'\i{}sica de Altas Enerx\'\i{}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain}

\author{D.~Zavrtanik}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}

\author{M.~Zavrtanik}
\affiliation{Experimental Particle Physics Department, J.\ Stefan Institute, Ljubljana, Slovenia}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{L.~Zehrer}
\affiliation{Center for Astrophysics and Cosmology (CAC), University of Nova Gorica, Nova Gorica, Slovenia}

\author{A.~Zepeda}
\affiliation{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico, D.F., M\'exico}

\collaboration{The Pierre Auger Collaboration}
\email{auger_spokespersons@fnal.gov}
\homepage{http://www.auger.org}
\noaffiliation


